Performance of the EDELWEISS-III experiment for direct dark matter searches

We present the results of measurements demonstrating the efficiency of the EDELWEISS-III array of cryogenic germanium detectors for direct dark matter searches. The experimental setup and the FID (Fully Inter-Digitized) detector array is described, as well as the efficiency of the double measurement of heat and ionization signals in background rejection. For the whole set of 24 FID detectors used for coincidence studies, the baseline resolutions for the fiducial ionization energy are mainly below 0.7 keV$_{ee}$ (FHWM) whereas the baseline resolutions for heat energies are mainly below 1.5 keV$_{ee}$ (FWHM). The response to nuclear recoils as well as the very good discrimination capability of the FID design has been measured with an AmBe source. The surface $\beta$- and $\alpha$-decay rejection power of $R_{\rm surf} < 4 \times 10^{-5}$ per $\alpha$ at 90% C.L. has been determined with a $^{210}$Pb source, the rejection of bulk $\gamma$-ray events has been demonstrated using $\gamma$-calibrations with $^{133}$Ba sources leading to a value of $R_{\gamma{\rm -mis-fid}} < 2.5 \times 10^{-6}$ at 90% C.L.. The current levels of natural radioactivity measured in the detector array are shown as the rate of single $\gamma$ background. The fiducial volume fraction of the FID detectors has been measured to a weighted average value of $(74.6 \pm 0.4)\%$ using the cosmogenic activation of the $^{65}$Zn and $^{68,71}$Ge isotopes. The stability and uniformity of the detector response is also discussed. The achieved resolutions, thresholds and background levels of the upgraded EDELWEISS-III detectors in their setup are thus well suited to the direct search of WIMP dark matter over a large mass range.

==> setup.tex <==
\section{Experimental setup}

\subsection{Cryogenics}
    Dilution refrigerator. Base temperature. Temperature screens. 
    \textbf{ALEX NOTE : VERSION 0}

The EDELWEISS-III cryostat is a custom-made cryostat. It is based on the \EDD\ cryostat that was running at the Laboratoire Souterrain de Modane (LSM) from 2005 to 2012. The EDELWEISS-II cryostat has then been modified essentially to improve the microphonics level, to decrease the 50K and 100K stages temperature to improve ionization resolution and to decrease the Helium consumption.
A key feature of this cryostat is its reversed geometry with the dilution unit at the bottom and the detector volume at the top of the cryostat.
The whole cryostat is isolated by four active pneumatic isolators controlled by a PID loop, which act as a low-pass filter (> 1 Hz). 
The 100K and 50K screens are cooled in serie by a cold He4 gas cryoline at 2 bars. This cryoline is cooled by two Gifford Mac-Mahon two stages thermal machines. \textbf{(200W at 50K ?)} The cryoline allows a full mechanical decoupling of the cold heads from the cryostat.
The Temperature of the He4 gas at 2b is at about 40K at the entrance of the 50K screen and 80K at the output of the 100K screen. He4 pressure and mass flow could be controlled to stabilize the 50K and 100K screen. Running temperatures are at about 50-55K and 85-90K.
The 4K screen is cooled by the cold vapor of liquid He4 evaporation.
This liquid Helium consumption is reduced close to 0 by the use of a cold vapor reliquefaction system, based on a third  Gifford Mac-Mahon machine with a cooling power of 1.5 W at 4.2 K. 
The whole 1K stage is tightly isolated from the main cryostat vacuum. This stage is cooled by a 1K pot controlled by a cold valve connected to the  $^{4}$He bath.
In the standard conditions the He consumption is roughly 100 liters per week.
 A global view of the cryostat is shown in Fig~\ref{fig:CryoEDWIII}


\begin{figure}
\begin{center}
\includegraphics[width=1\textwidth]{figures/CryoEDWIII.png}
\end{center}
\caption[]{Cross-section of the EDELWEISS-III reversed cryostat connected with its 3 thermal machines with a cryoline. A part of the Pb-shielding (orange) is shown. The He dewar is the structure at the bottom.}
\label{fig:CryoEDWIII}
\end{figure}



\subsection{Shields}
   Pb shields.  PE shields. 
   
   \textcolor{red} {Figure: GEANT4 geometry plot?}
\begin{figure}
\begin{center}
\includegraphics[width=1\textwidth]{figures/CryoEDWIII.png}
\end{center}
\caption[]{General setup of \EDDD (correct figure to be included!)}
\label{fig:EDWIIIsetup}
\end{figure}
   
   \textcolor{red} {text below copied from muon bgd paper}   
The outermost layer of the \EDW\ setup is the $\mu$-veto system, a layer of plastic scintillator acting as an active shield to tag any muon-induced activity in the bolometer system. It consists of 46 individual plastic scintillator modules (Bicron BC-412) of 65\,cm width, 5\,cm thickness and lengths of 2\,m, 3.15\,m, 3.75\,m and 4\,m adding up to a total surface of 100\,m$^2$. The modules are assembled in a stainless steel mounting frame and attached to the PE shielding to ensure an almost hermetic coverage of the experiment setup. Due to the need for access to the cryostat during maintenance intervals, parts of the \muveto are positioned on rails on top of the two movable PE blocks to allow a roll-back during cryostat access (Fig.~\ref{fig:EDWIIIsetup}). Whereas the upper level (N1) of the \muveto almost completely covers the PE shielding, except for small openings for rails, the part below the cryostat level (N0) has more prominent gaps due to the cryogenic supply lines, and the pillars on which the 
entire experiment is mounted. The overall geometrical muon flux coverage of the \muveto amounts to 98\%. To ensure proper closure during data taking, the exact positions of the two mobile veto parts are monitored via regular position measurements using laser interferometry.

Each module is viewed by two groups of four 2-inch PMTs (Philips Valvo XP2262/PA). Each group has an individual high voltage (HV) supply and readout, leading to a total of 92~HV and signal channels. The data acquisition is based on VME electronics with special cards developed in-house. An event recording in the veto system is triggered once the two signals of a module each pass a trigger threshold within a coincidence window of 100\,ns. With leading edge discriminators set at the same level of 150\,mV, individual modular thresholds are achieved by adjusting the HV values. Within an event, all hits above threshold in the modules are then registered within an interval of $\pm125$\,ns around the trigger time. For each signal channel, the individual time of a hit is recorded in a 128-channel TDC (CAEN V767) and the analog signals are converted in three 32-channel QDCs (CAEN V792). After the coincidence window, any further input is blocked for about 50\,$\mu$s until the event data are read out via the VME bus and all active elements are reset by the acquisition software. The time information with respect to the bolometers is received via an optical fiber which transmits the 10\,$\mu$s time stamp in 48 bits of 64\,ns width each. This sequence of bits is converted via an FPGA-based board and then read out via the VME bus. To monitor the overall status of the veto modules, the hit rate of all PMT groups (not requiring any coincidence) is recorded in scalers. These data are processed continuously to check the performance of the \muveto via a graphical web interface.

A muon traversing a scintillator module as a minimal ionizing particle deposits on average more than 10\,MeV. The average energy deposition is 11.8\,MeV for horizontal modules on the top and bottom, and up to 24\,MeV for modules on the sides. These values are above typical energy deposition from the ambient radioactivity. For each channel, the energy deposition is stored as the integrated charge Q in units of ADC values. With the comparison of the Landau most probable values (MPV) of the integrated charge Q of specific two module coincidence cuts with dedicated MC simulations, a module-individual calibration is obtained with a mean calibration coefficient of 5.44\,keV/ADC-value. The effective threshold of the muon veto modules has been chosen to be much lower than the MPVs (about 5\,MeV at the center of a module, rising towards the module ends due to the position-dependent light 
output) to be also able to detect grazing muons and thus to keep the muon detection efficiency as high as possible. As a result, the rate of recorded events in the entire system is of the order of one per second, to be compared to an expected rate of throughgoing muons hitting at least one module per system section N1 and N0 of $\sim 3.5\times 10^{-4}$\,Hz. Whereas the rate of recorded events is dominated by ambient background, candidates of throughgoing muons can be easily extracted from the data by requiring two modules in coincidence.

More details on the \muveto and on the measured muon flux can be found in \cite{muonveto}.
   
